CompeteAI: Understanding the Competition Dynamics in Large Language Model-based Agents

Large language models (LLMs) have been widely used as agents to complete different tasks, such as personal assistance or event planning. While most of the work has focused on cooperation and collaboration between agents, little work explores competition, another important mechanism that promotes the development of society and economy. In this paper, we seek to examine the competition dynamics in LLM-based agents. We first propose a general framework for studying the competition between agents. Then, we implement a practical competitive environment using GPT-4 to simulate a virtual town with two types of agents, restaurant agents and customer agents. Specifically, the restaurant agents compete with each other to attract more customers, where competition encourages them to transform, such as cultivating new operating strategies. Simulation experiments reveal several interesting findings at the micro and macro levels, which align well with existing market and sociological theories. We hope that the framework and environment can be a promising testbed to study competition that fosters understanding of society. Code is available at: https://github.com/microsoft/competeai.

==> related_work_previous_version.tex <==

\textbf{Cooperation and competition.}
Empirical studies have provided valuable insights into the dynamics of cooperation and competition~\citep{porter2008competition, kosfeld2011competition}. For instance,~\citet{markussen2014competition} found that inter-team competition can serve as a catalyst for intra-team cooperation by stimulating improvements in relative group performance. \citet{chen2008reconceptualizing} further highlighted the intricate interplay between cooperation and competition in real-world scenarios. 
In AI and computer science, there exists a substantial body of literature dedicated to investigating cooperation and competition in simulated environments~\citep{dafoe2020open, drury2009cooperation}. \citet{castelfranchi1998modelling} introduced a framework for modeling social environments using AI agents, encompassing elements such as cooperation, groups, and organizations. Building upon this foundation, \citet{dafoe2020open} and \citet{zhang2023proagent} proposed open problems in cooperation AI, aiming to enhance the joint welfare of a group, thereby contributing to the understanding of these dynamics in artificial environments. 
In our work, we leverage LLM-based agents, known for their profound natural language understanding and reasoning capabilities, to effectively stimulate human behaviors and probe the intricate interactions within a novel \textit{competition} scenario.
Moreover, our work distinguishes itself from recent contributions such as~\citet{chen2023money} by introducing a versatile competition framework adaptable to diverse competitive situations.
Preliminaries of theories can be found at \cref{sec-append-pre}.


% Large language models (LLMs)~\citep{openai2023gpt4, touvron2023llama, zeng2023glm-130b} attracted considerable attention owing to their exceptional proficiency in a wide range of natural language understanding and generation tasks~\citep{wang2023robustness, xiao2023large, chen2023semi, zhou2023synthetic, li2023emotionprompt}. 
\textbf{Large language models as agents.}
There has been a burgeoning area of research that utilizes LLMs as central controllers to create autonomous agents capable of human-like decision-making~\citep{wang2023survey,xi2023rise, huang2023benchmarking, wang2023voyager,li2023metaagents, chang2023survey}. 
Studies have indicated that while exhibiting effective experiential learning~\citep{zhao2023expel}, leveraging multiple LLMs through cooperation and debate can further enhance their capabilities~\citep{abdelnabi2023llm}. This is achieved by integrating multiple LLMs into a cohesive group and designing specific interaction mechanisms. For instance, AutoGen~\citep{wu2023autogen} introduces a novel framework that facilitates the development of LLM applications using multiple customizable, conversational agents capable of collaborative problem-solving. The applications are diverse, including task planners~\citep{wang2023describe, song2023llm}, simulators in behavioral economics studies~\citep{horton2023large}, and judges in specific domains~\citep{chan2023chateval}.
Our work primarily investigates agents' behaviors in competition scenarios, an area that has received relatively less attention but holds equal significance.

% Moreover, our work contributes to the evaluation protocols of LLM-based agents by emphasizing a unique aspect. Instead of relying solely on quantitative metrics~\citep{liu2023agentbench, jin2023better}, our evaluation methodology is naturally inspired by classic sociological and economic theories that prioritize a careful interaction process and meticulous observations to assess these agents' performance. This detailed and iterative process may also trigger new interest in future research on LLM-based agents.



% The relationship between cooperation and competition has been a long-standing subject of research in the fields of economics, biology, and social sciences~\citep{stapel2005competition, khanna1998dynamics, luo2022relationships, deutsch2011cooperation}. 
% This relationship has been explored through a combination of empirical studies and agent-based simulations. 


% \section{基于大语言模型的代理建模研究}
% \label{sec-related-work-llms4abm}

% 由于大语言模型（LLMs）展现出了强大的能力和类人的行为，众多研究人员开始将基于LLMs构建的代理应用于ABM领域，以期构建更智能的代理和更真实复杂的模拟场景。
% 其中，Generative Agents~\citep{park2023generative} 作为一项开创性的工作，构建了一个包含25个代理的村庄。研究人员系统地设计了模拟环境中代理的架构，为后续代理架构设计奠定了基础。同时，他们利用该模拟环境探讨了信息传播现象与机制，开辟了基于LLMs的代理在ABM中应用的先河。
% RecAgent~\citep{wang2024user}构建了一个虚拟的推荐系统环境，并利用该环境探究了信息茧房和用户从众行为。
% EconAgent~\citep{li2024econagent}将基于LLMs的代理应用于宏观经济学环境中，并成功还原出传统模拟方法未能还原出的真实现象。

% 在协同合作领域，也有诸多研究成功。
% CAMEL~\citep{li2023camel}提出了一个代理合作框架，其中包括负责规划命令的指挥者和负责执行任务的执行者。
% ChatDev~\citep{qian2023communicative}设计了一家虚拟软件公司，为其中的代理赋予CEO, 工程师等各种角色。代理们合作完成软件的开发。
% \citet{zhang2023exploring} 系统探究了代理间的合作机制，并从社会心理学的角度进行了阐释。
% 然而，与合作同等重要的竞争机制却鲜有研究。
% \citet{chen2023money}构建了拍卖这一竞争场景，但其重点在于评估LLMs在竞争中规划执行的能力，而非分析LLMs表现出的行为和系统的动态变化；\citet{han2023guinea} 研究了公司竞争和合作，但仅关注价格动态变化。这些研究都缺乏对复杂竞争环境模拟和对竞争行为和系统演变的探究，我们的工作弥补了这一缺陷。



